Improving Health Professionals' Onboarding with AI and XAI for Trustworthy Human-AI Collaborative Decision Making

With advanced AI/ML, there has been growing research on explainable AI (XAI) and studies on how humans interact with AI and XAI for effective human-AI collaborative decision-making. However, we still have a lack of understanding of how AI systems and XAI should be first presented to users without technical backgrounds. In this paper, we present the findings of semi-structured interviews with health professionals (n=12) and students (n=4) majoring in medicine and health to study how to improve onboarding with AI and XAI. For the interviews, we built upon human-AI interaction guidelines to create onboarding materials of an AI system for stroke rehabilitation assessment and AI explanations and introduce them to the participants. Our findings reveal that beyond presenting traditional performance metrics on AI, participants desired benchmark information, the practical benefits of AI, and interaction trials to better contextualize AI performance, and refine the objectives and performance of AI. Based on these findings, we highlight directions for improving onboarding with AI and XAI and human-AI collaborative decision-making.

==> figures/figure_tutorial.tex <==


\begin{figure*}[htp]
\centering 
\begin{subfigure}[t]{0.51\textwidth}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/3_tutorial_ai.png}
  \caption{}
  \label{fig:tutorial_ai}
\end{subfigure}\hspace{5mm}
\begin{subfigure}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/4_tutorial_data.png}
  \caption{}
  \label{fig:tutorial_data}
\end{subfigure}
\begin{subfigure}[t]{0.51\textwidth}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/5_tutorial_performance.png}
  \caption{}
  \label{fig:tutorial_performance}
\end{subfigure}\hspace{5mm}
\begin{subfigure}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/6_tutorial_xai.png}
  \caption{}
  \label{fig:tutorial_xai}
\end{subfigure}
\begin{subfigure}[t]{0.51\textwidth}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/7_tutorial_feat.png}
  \caption{}
  \label{fig:tutorial_feat}
\end{subfigure}\hspace{5mm}
\begin{subfigure}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/8_tutorial_counter.png}
  \caption{}
  \label{fig:tutorial_counter}
\end{subfigure}
\begin{subfigure}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/9_tutorial_example.png}
  \caption{}
  \label{fig:tutorial_example}
\end{subfigure}
\caption{Onboarding Tutorial Materials of an AI: (a) and (c) the context of hysical Stroke Rehabilitation Assessment:, (b) AI applications of the , (d) a diagram of how AI is developed and operates, (e) dataset, (f) evaluation metrics and performance, (g) motivation of an AI explanation, (h) a feature importance explanation, (i) a counterfactual explanation, and (j) prototype/example-based explanations.}\label{fig:tutorials}
\end{figure*}


==> tables/trustworthy_relationship.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\caption{Process to Build a Trustworthy Relationship with Colleagues and Characteristics of a Trustworthy Colleague}
\label{tab:trustworthy_relationship}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{lll} \toprule
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Process to Build a\\ Trustworthy Relationship\end{tabular}} &
  \multicolumn{2}{c}{Characteristics \& Factors} \\ \midrule
Interactive Communications &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Soft Skills: \\ “Being honest”, “Approachable \& Friendly”, “Timeliness”\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}“Reputation with others”\\ “Confidentiality”\end{tabular}} \\ \cline{1-2}
Adding a Value &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}“Having expertise”\\ “Provide sound, consistent, and reliable facts”\end{tabular}} & \\ \bottomrule
  
\end{tabular}%
}
\end{table}
